Dynamic Graph-Based Anomaly Detection in the Electrical Grid

Given sensor readings over time from a power grid, how can we accurately detect when an anomaly occurs? A key part of achieving this goal is to use the network of power grid sensors to quickly detect, in real-time, when any unusual events, whether natural faults or malicious, occur on the power grid. Existing bad-data detectors in the industry lack the sophistication to robustly detect broad types of anomalies, especially those due to emerging cyber-attacks, since they operate on a single measurement snapshot of the grid at a time. New ML methods are more widely applicable, but generally do not consider the impact of topology change on sensor measurements and thus cannot accommodate regular topology adjustments in historical data. Hence, we propose DYNWATCH, a domain knowledge based and topology-aware algorithm for anomaly detection using sensors placed on a dynamic grid. Our approach is accurate, outperforming existing approaches by 20% or more (F-measure) in experiments; and fast, running in less than 1.7ms on average per time tick per sensor on a 60K+ branch case using a laptop computer, and scaling linearly in the size of the graph.

==> 010introduction.tex <==
Maintaining as well as improving the reliability of power delivery is a critically important goal. Estimates~\cite{amin2011us} suggest that reducing outages in the U.S. grid could save $\$ 49$ billion per year, reduce emissions by $12$ to $18\%$, while improving efficiency could save an additional $\$ 20.4$ billion per year \reminder{cite works}. Although, many practices exist today that work to maintain the reliability of the electric grids, a new form of the adversary in the form of cyber-intrusion is emerging and is becoming a growing concern. This is evident from the reports of foreign hackers successfully penetrating control rooms of U.S. power plants~\cite{perlroth2017hackers} and of cyber-attacks targeted toward Ukrainian grid in 2015-2016 \reminder{cite} that brought down sections of the grid causing damages worth billions of dollars. This in addition to natural failures of grid equipment and measuring devices remain to be a problem that grids of today must face \reminder{cite}.\par

One of the most key elements of maintaining grid reliability is the ability to maintain accurate situational awareness in the control room. Loss of or even worse comprised situational awareness in the control room can severely disrupt the operation of the grid. Situational awareness amongst other things is most dependent on the network topology and grid measurements. Errors or anomalies either due to natural failures and intentional attacks within these can impact it. A key component to safeguard against this is to use the growing network of sensors in conjunction with anomaly detection techniques to quickly identify when network topology or grid measurements are anomalous, so as to quickly respond to the problem in real-time. Most common amongst these are by processing the measurement data and network topology to detects anomalous behavior, leveraging different types of data behavior patterns extracted from the processed data values, dynamics, and other feature characteristics. Generally, these spatial and temporal patterns of data can be sourced from either normal or abnormal events. 
Examples of normal events during regular operation and control include 

\begin{itemize}
    \item Regular power configuration adjustments, i.e., change of load and generation,
    \item Regular system topology change: transmission line / transformer on/off, bus split, shunt switching.
\end{itemize}
On the other hand, examples of abnormal events include: 
\begin{itemize}
    \item False measurements which range from traditional bad data to targeted false data injection caused by cyber-attacks, etc, 
    \item Topological error: unwanted topological change due to unexpected component failures, natural disasters, physical attacks, etc,
    \item Others faults and anomalies.
\end{itemize}

For any method aiming at anomaly detection in grid measurements and topology, the essential capability is to identify abnormal events while accommodating regular behaviors. Today this functionality is achieved through Energy Management Systems (EMS) within the control rooms. These collect various sources of data: measured data from remote terminal units (RTUs) and phasor measurement units (PMUs) and corresponding grid topology from communication channels coming through Supervisory Control and Data Acquisition System (SCADA). Processing and analyses of this data through methods such as AC State-Estimation (ACSE) and topology estimator (TE) serves as the basis for detecting any anomalies in the grid measurement or topology.

\reminder{Talk about problems with existing ACSE and TE in terms of anomaly detection}
First, we briefly discuss ACSE and its bad-data detection capabilities. In the bulk energy system (BES), ACSE runs every 5 to 15 minutes, along with its bad data detection (BDD) and identification (BDI) algorithm. It inputs analog measurements and an estimated topology to output the most likely grid state by solving an optimization problem and traditionally whose residuals are further used for BDD and BDI via hypothesis test and other statistical methods. The most widely used problem formulation is the weight-least-square (WLS) form, minimizing the least mean square of measurement error. Some other formulations are designed with intrinsic robustness against bad data, including least absolute value (LAV) based, least median of squares based, as well as iteratively reweighted least-squares based approaches. Unfortunately, these methods generally suffer from difficult convergence due to nonlinear measurement models. To handle the nonlinearity, some recent methods have been developed for convexification of the optimization problem: [xx] reduces the problem to an equality-constrained QP by creating linear measurement models through a mapping of input measurements based on sensitivity.  [xx] convexifies the problem by reformulating the $|V|$, phase angle, as well as the product of voltage and current, in SDP form, through matrix transformation. These convexification techniques improves convergence, yet several limitations still exist in SE BDD/BDI:
\begin{itemize}
    \item Only applicable to traditional bad data but not coordinated attacks like a well-crafted false data injection attack (FDIA) where measurement values are maliciously altered in a way that state estimation result deviates largely from the truth but the residual remains small and fails to indicate the existence of attack.
    \item Highly sensitive to network topology and fails when a good topology of the grid is not available. Any erroneous topology can manifest itself as multiple bad data and confuse the SE BDD/BDI.
\end{itemize}

\reminder{Following paragraph has a lot of citations missing.}
Particularly, the assumption of accurate topology in SE raises the need for reliable topology estimation as another EMS function. The conventional topology estimator, also known as network topology processor (NTP), processes the input circuit breaker/switching status and transforms the bus-section-switching model into the bus-branch model, with network connectivity and meter locations determined. However, the conventional NTP always assumes the input status data are correct. Topological errors due to communication, operator entry errors, cyber-attacks and any faults not reflected on circuit breaker/switching status can pass undetected throughout the analysis. To handle this, generalized topology processing, also called generalized state estimation, has been developed where pseudo measurements are created and a DC SE is performed on the small sub-network within a suspicious substation, followed by a hypothesis test. Another type of approach is to apply a hypothesis test on WLS residuals from SE to detect topological errors, as an extended application of SE BDI. In recent years, advanced methods have been developed where TE and SE are merged together by performing ACSE on the entire network using a bus-breaker model. This enables measurement error and topology error to be effectively identified and separated. However, similar troubles remain for TE. On the one hand, convex formulations for TE or merged TE-SE for AC power systems are not well developed, making the existing approaches inefficient. And on the other hand, the inability to handle complex errors, like those caused by cyber-attack, still exists.

\reminder{This para talks about Defined behavior $\longrightarrow$ statistical behavior:}
Clearly, some effort is needed to handle the remaining challenges. 
Considered from the detection mechanisms, a major cause is that the existing TE and SE BDD/BDI only capture some defined data behaviors, using the well-defined measurement models in state estimation, and information in these behaviors are limited to a snapshot \textcolor{red}{Describe snapshot more clearly}. Later with the popularity of machine learning techniques, statistical behaviors have been widely explored and captured \reminder{citations missing. transactions require very thorough existing work. that is missing here}, managing to extract useful temporal patterns from historical data. The leveraging of statistical behavior resolves some issues above, since most anomalies, either unexpected faults or cyber-attacks, usually disrupt the statistical consistency of the data stream, despite being invisible from one snapshot. The incorporation of machine learning also gives rise to advanced SE architectures with anomaly detection serving as a supplementary module to validate the SE solution.

\reminder{this para is about ML without topology}
\reminder{this para is about ML with static topology}

Existing behavioral anomaly detection methods can be broadly categorized into model-based (where an expectation of observation is obtained by fitting a mathematical model), representation-based, graphical methods, etc. %More detailed classifications can be found in xxx. 
Generally, these families of the method are all applicable to the problem in this paper. Moreover, with input data recorded in an orderly fashion and correlated across the spatial graph, applying ML methods in time series and graph context is a good way to extract meaningful knowledge. A short review of relevant approaches is given in section \ref{sec:relatedwork}. 

However, when treating the multivariate input, few methods have explored the impact of graph change on the observations. Existing methods either ignore the impact of graph topology in their detection or assume a static topology across the data stream. This can be problematic. Since different grid configurations naturally cause differences in grid measurements, previous observations from disparate topologies may provide little value in assessing the anomalousness for now. Without a selection of relevant data, methods can include more false positives by falsely creating alarms when regular topology changes occur. 

For purposes of behavioral analysis, a more applicable method is a context-aware analysis which indicates the expected patterns of behavior from data samples collected with relevant context of topology. Here our paper proposes a method that processes the time series of measurements and the time series of topology. Intuitively, the method works by defining graph distances and estimating the most reliable distribution of measurement at a specific time t, so that an alarm is created if the measured value deviates largely from the center of the distribution. The goal of the method is to
\begin{itemize}
    \item Detect false measurement due to bad data or false data injection attack.
    \item Detect topological error. Any topological anomaly undetected in TE will trigger an alarm.
    \item Directly consider the impact of topology on the estimation of the measurement value, so that any topology change in previous data is allowed.
\end{itemize}
 
Further, to account for the large-scale grid, we develop a local-sensitive version Dynwatch-local.  

%Table X shows a comprehensive comparison of detection capabilities for different families of methods.
\reminder{explain why we didn't discuss load and generation change} Here, big and abrupt changes in load and generation are not discussed in our paper. Typically under normal conditions, the power configuration of today’s power grid is still expected to change gradually, as the quasi-steady-state (QSS) model assumes. Yet unstable behaviors can also happen, especially when high penetration of distributed energy resources causes problems. For any existing method trying to check statistical consistency, an unstable power configuration, if any, should be flagged as an anomaly when it disturbs the temporal pattern of the analyzed data. 

%The paper is structured as follows:


==> 011introduction_R1.tex <==
\reminder{Para 1:Introduction to power grid reliability and need for anomaly detection}
Maintaining and improving the reliability of the electric power grid is a critically important goal. Estimates~\cite{amin2011us} suggest that reducing outages in the U.S. grid could save $\$ 49$ billion per year, reduce emissions by $12$ to $18\%$, while improving efficiency could save an additional $\$ 20.4$ billion per year. Although grid operators and engineers work tirelessly to maintain reliability of the electric grids, many challenges persist. Climate change is increasing the frequency of natural disasters, resulting in higher failure rate of grid equipment including sensing devices. Also, there is an emergence of a new adversary in the form of cyber-intrusions that targets electric grid reliability through disrupting the control and communication layer. This is evident from the reports of foreign hackers successfully penetrating control rooms of U.S. power plants~\cite{perlroth2017hackers} and of cyber-attacks targeted toward Ukrainian grid in 2015-2016 \cite{ukrain2015}\cite{lee2017crashoverride} that brought down sections of the distribution network causing damages worth billions of dollars.  

%One of the most key elements of maintaining grid reliability is the ability to maintain accurate situational awareness in the control room. Loss of or even worse comprised situational awareness in the control room can severely disrupt the operation of the grid. Situational awareness amongst other things is most dependent on the network topology and grid measurements. Errors or anomalies either due to natural failures and intentional attacks within these can impact it. 
\reminder{Para2:Fundamentals and very brief state-of-the-art for anomaly detection algorithms}
A key tool that the grid operators have for safeguarding against these failures, whether naturally occurring or malicious, are the anomaly detection methods that are implemented in grid control rooms. These help grid operators isolate faulty data from the healthy ones to result in accurate situational awareness, which further allows grid operators to take corrective actions in real-time. Broadly, these methods analyze grid measurement values, dynamics and other informative features to detect abnormal events, including erroneous topology or measurements, while accommodating normal grid behaviors which are regular topology changes and power configuration adjustments.

%%no longer used
% \reminder{I think you can combine all the lines within the dashed lines to simply explain anomaly detection for power grids and what kind of data it works on. Just a line or two}

% \\----------------
% These methods identify any anomalous measurement data or topology status based on prior collected data, so as to quickly respond to the problem in real-time. \reminder{Combined the next two lines to say something that flows with the paragraph}
% Presently, general anomaly detection techniques leverage different types of data behavior patterns extracted from the processed data values, dynamics, and other feature characteristics. For any method aiming at anomaly detection in grid measurements or grid topology, the necessary requirement is to identify abnormal events while accommodating the regular behaviors. 

% Generally, the spatial and temporal patterns of data, can be sourced from either normal or abnormal events. 
% Examples of normal events, during regular operation and control, include regular power configuration adjustments and topology changes.
% On the other hand, examples of abnormal events include topological error, false measurements and other anomalies. 
% -----------\\

\reminder{Para3: Anomaly detection in power grids today. Describe and define the two sets of data: measurement data and device indicators. Mention separate anomaly detection method is used for each set of data.}
In existing power grids, anomaly detection is performed within the Energy Management Systems (EMS) \cite{EMS} that are installed in the control rooms. The EMS through Supervisory Control and Data Acquisition (SCADA) system collects two primary sources of data: i) online measurement data from various sensors such as remote terminal units (RTUs) and phasor measurement units (PMUs) and ii) status indicators for various devices such as lines and transformers. Together these two classes of data provide sufficient information for reliable and secure operation of the grid. To find anomalous data in these two classes of data, two separate analyses within the EMS are run. 

\reminder{Para 4: Describe ACSE+BDD. Problems with that.}
AC state-estimation \cite{WLS-SE} along bad-data detection algorithms \cite{traditional-BDI} provide anomaly detection for measurement data from RTUs and PMUs. These  are run  every 5 to 15 minutes 
%. It inputs analog measurements and an estimated topology to output the most likely grid state 
by solving an optimization problem and traditionally whose residuals are further used for BDD and BDI via hypothesis test and other statistical methods. The most widely used problem formulation is the weight-least-square (WLS) form\cite{traditional-BDI}, minimizing least mean square of measurement error. Some other formulations are designed with intrinsic robustness against bad data, including least absolute value (LAV) based \cite{LAVSE-PMU-abur}, least median of squares based \cite{robustSE-median}, as well as iteratively reweighted least squares based approaches \cite{robustSE-reweight}. Unfortunately, these methods generally suffer from difficult convergence due to nonlinear measurement models. 
%To handle the nonlinearity, 
Some recent methods developed for convexification of the optimization problem\cite{convexSE-LAV-Li}\cite{convexTESE-SDP-weng}\cite{SUGAR-SE-Alex}\cite{SUGAR-SE-Li} 
%: [xx] reduces the problem to an equality-constrained QP by creating linear measurement models through a mapping of input measurements based on sensitivity.  [xx] convexifies the problem by reformulating the $|V|$, phase angle, as well as product of voltage and current, in SDP form, through matrix transformation. 
resolved the convergence issues, yet several limitations still exist in SE BDD/BDI:
\begin{itemize}
    \item Only applicable to traditional bad data but not coordinated attacks like false data injection attack (FDIA)\cite{fdia-review}% where measurement values are maliciously altered in a way that state estimation result deviates largely from truth but the residual remains small and fails to indicate the existence of attack
    \item Highly sensitive to network topology:
    Any erroneous topology can manifest itself as multiple bad data and confuse the SE BDD/BDI
\end{itemize}

%
\reminder{AP Example of how this paragraph should look like..}
\textcolor{red}{On the other hand, topology anomalies are detected by network topology processor (NTP)\cite{TE-NTP-book}\cite{TE-NTP-tracking}, which transforms the input circuit breaker/switching status data into bus-branch model, with network connectivity and meter locations determined. However, NTP does not account for topological errors due to communication, operator entry errors, cyber-attacks or faulty data. To handle this, generalized topology processing \cite{TE-GSE} was developed that uses pseudo-measurements and hypothesis test to detect topology anomalies. Another approach \cite{TE-WLSE-BDI} applies hypothesis test on WLS residuals from SE to detect topological errors, as an extended application of SE BDI. More recently, other advanced methods such as \cite{TESE-GSE}\cite{TESE-GSE-PMUabur}\cite{convexTESE-SDP-weng} have been developed where TE and SE are merged together to perform ACSE using a bus-breaker model. This enables measurement error and topology error to be effectively identified and separated. However, challenges corresponding to the traditional ACSE problem persist here as well. Majority of these approaches are formulated as non-convex options that are prone to divergence and long run-times. Furthermore, none of them are designed to detect anomalies due to coordinated attacks such as those originating from cyber-intrusions.}

\reminder{Para 6: Describe your approach. Finish with contributions}
The existing challenges suggest a gap in research community that is able to accurately detect anomalies in both topology as well as measurement data. 
%Considered from the detection mechanisms, a major cause is that the existing TE and SE BDD/BDI only capture some defined data behaviors, using the well-defined measurement models in state estimation, and information used for checking these behaviors is limited to a snapshot, without looking at previous time frames. Later with popularity of machine learning techniques, statistical behaviors have been widely explored and captured, managing to extract useful temporal patterns from historical data\cite{hooi2018gridwatch}\cite{keogh2007finding}\cite{breunig2000lof}\cite{yi2017grouped}. The leveraging of statistical behaviors resolves some issues above, since most anomalies, either unexpected faults or cyber attacks, usually disrupt the statistical consistency of the data stream, despite being invisible from one snapshot. %The incorporation of machine learning also gives rise to advanced SE architectures with anomaly detection serving as a supplementary module to validate the SE solution.
Having a behavior-based anomaly detector as a supplementary to TE and SE can help resolve some issues above. Instead of analysing the well-defined measurement models in a snapshot, the leveraging of statistical behaviors extracts some patterns from historical data. This can be helpful since since most anomalies, either unexpected faults or cyber-attacks, usually disrupt the statistical consistency of the data stream, despite being invisible from one snapshot.

Existing behavioral anomaly detection methods can be broadly categorized into model-based (where an expectation of observation is obtained by fitting a mathematical model)\cite{hamilton1994time}\cite{regression4AD}\cite{yi2017grouped}, representation based\cite{breunig2000lof}\cite{LOFvariants}, graphical methods\cite{liu2008isolation}, etc. 
Generally, these families of method are all applicable to the problem in this paper. Moreover, with input data recorded in an orderly fashion and correlated across the spatial graph, applying ML methods in time series and graph context is a good way to extract meaningful knowledge. A short review of relevant approaches is given in section \ref{sec:relatedwork}. 

However, when treating the multivariate input, few methods have explored the impact of graph change on the observations. Existing methods either ignore the impact of graph topology in their detection\cite{hamilton1994time}\cite{yi2017grouped}\cite{breunig2000lof}, or assume a static topology across the data stream\cite{hooi2018gridwatch}. This can be problematic. Since different grid configurations naturally cause differences in grid measurements, previous observations from disparate topologies may provide little value in assessing the anomalousness for now. Without a selection of relevant data, methods can include more false positives by falsely creating alarms when regular topology changes occur. 

To handle this, a more applicable method is a context-aware analysis which indicates the expected patterns of behavior from data samples collected with relevant context of topology. Here our paper proposes such a method that processes the time series of measurements and the time series of topology. Intuitively, the method works by defining graph distances and estimating a reliable distribution of  measurement at time $t$ from the most relevant previous data. And finally an alarm is created if the measured value deviates largely from the center of distribution. The goal of the method is to directly consider the impact of topology on observations, so that regular topological changes are accommodated, while detecting any false measurement and topological errors.
Further, to account for large-scale grid, we develop a local-sensitive version Dynwatch-local.  

%\reminder{not sure if this para is needed}In addition, big and abrupt changes on load and generation are not discussed in our paper. Typically under normal conditions, the power configuration of today’s power grid is still expected to change gradually, as the quasi-steady state (QSS) model assumes. Yet unstable behaviors can also happen, especially when high penetration of distributed energy resources causes problems\cite{violateQSS}. For any existing method trying to check statistical consistency, an unstable power configuration, if any, should be flagged as an anomaly when it disturbs the temporal pattern of the analysed data. 

The rest of the paper is organized as follows: Section \ref{sec:relatedwork} provides background of existing methods. Section \ref{sec:method} shows our proposed method. Section \ref{sec:Results} validates the method with experiment results. Finally, Section \ref{sec:Conclusion} concludes the paper.
